Autonomous Recognition of Erroneous Raw Key Bit Bias in Quantum Key Distribution

As Quantum Key Distribution technologies mature, it is pertinent to consider these systems in contexts beyond lab settings, and how these systems may have to operate autonomously. To begin, an abstract definition of a type of error that can occur with regard to the ratio of bit values in the raw key is presented, and how this has an impact on the security and key rate of QKD protocols. A mechanism by which errors of this type can be autonomously recognised is given, along with simulated results. A two part countermeasure that can be put in place to mitigate against errors of this type is also given. Finally some motivating examples where this type of error could appear in practice are presented to add context, and to illustrate the importance of this work to the development of Quantum Key Distribution technologies.

==> sections/introduction/pa.tex <==
\subsection*{Privacy Amplification}
\label{sec:intro_pa}

Once Alice and Bob have established their raw keys, they must consider the fact that some information may have been leaked to Eve.
To remove this leaked information, they can employ privacy amplification \cite{renner2008security}.

In order to do this, they must first consider how much information needs to be removed.
It has been shown that the length of the remaining key after privacy amplification can be bounded by:
\begin{equation}
    \label{eq:intro_pa_compr_amount}
    \ell\lessapprox H^\varepsilon_{min}(R_A|E)
\end{equation}
where $H^\varepsilon_{min}(R_A|E)$ is the $\varepsilon$-smooth min-entropy of Alice's raw key conditioned on Eve's information.
However, as Eve's information is unknown to Alice and Bob, they must approximate this quantity.
It is the fact that they must approximate this quantity, \hl{and that it is proportional to the entropy of the raw key}, that this work makes use of in the section on the consequences for the security of QKD.
